Learning Image-Conditioned Dynamics Models for Control of Under-actuated Legged Millirobots

Millirobots are a promising robotic platform for many applications due to their small size and low manufacturing costs. Legged millirobots, in particular, can provide increased mobility in complex environments and improved scaling of obstacles. However, controlling these small, highly dynamic, and underactuated legged systems is difficult. Hand-engineered controllers can sometimes control these legged millirobots, but they have difficulties with dynamic maneuvers and complex terrains. We present an approach for controlling a real-world legged millirobot that is based on learned neural network models. Using less than 17 minutes of data, our method can learn a predictive model of the robot's dynamics that can enable effective gaits to be synthesized on the fly for following user-specified waypoints on a given terrain. Furthermore, by leveraging expressive, high-capacity neural network models, our approach allows for these predictions to be directly conditioned on camera images, endowing the robot with the ability to predict how different terrains might affect its dynamics. This enables sample-efficient and effective learning for locomotion of a dynamic legged millirobot on various terrains, including gravel, turf, carpet, and styrofoam. Experiment videos can be found at https://sites.google.com/view/imageconddyn

==> 04_baseline_NOT_USED.tex <==
\section{Differential Drive Baseline Method}
\label{sec:dd}

%%SL.02.27: maybe move this into the experiments section? it seems like a lot of time to spend just describing a hand-designed baseline method
In this section, we present an instantiation of a common steering method used for robots with wheel or leg-like mechanisms on both sides, known as differential drive. We compare our learning-based method with this baseline method in the following results section.

In this control scheme, the turn rate $\omega_{\text{robot}}$ is proportional to the difference between left $\omega_l$ and right $\omega_r$ leg velocities. A differential drive controller assumes that the system behavior can be thought of as two wheels connected by a common axis: Here, moving the right wheel would turn the robot to the left, and moving the left wheel would turn the robot to the right. Note that this general idea of a difference in leg velocities translating to heading change of the entire system can be implemented in many ways, and we describe our implementation below merely as a guideline.

As described in Algorithm.~\ref{alg:dd}, our implementation of a differential drive controller uses robot heading, as well as perpendicular distance away from the desired path, in order to set velocity setpoints for each side of robot. In addition to standard heading control where the robot turns such that its heading matches the angle of the line, it also incorporates the perpendicular error metric to say that its heading should be more or less than the heading of the line, in order to actually move back toward the line. This controller outputs desired leg velocities at a rate of 10 Hz. To enable the realization of these leg velocities, we also implement a low-level PID controller that runs in the firmware at 1000 Hz. Encoder readings of the leg positions provide feedback, and the PID controller monitors proportional, integral, and derivative errors in order to output the PWM values required for achieving the desired leg velocities.

\begin{algorithm}
  \caption{A Differential Drive Algorithm\\for Trajectory Following}
  \label{alg:dd}
\begin{algorithmic}[1]
    \STATE \textbf{Inputs}: Current state $(x,y,z,\text{roll},\text{pitch},\text{yaw})$, \\ \hspace*{35pt}Desired waypoints $W= [w_0, w_1, \dots]$, \\ \hspace*{35pt}Controller parameters $f1$ and $f2$
    \STATE Line segment $L \leftarrow$ closest $[w_i,w_{i+1}]$ to $(x,y)$
    \STATE $d_{\text{line}} \leftarrow$ angle of $L$
    \STATE $p \leftarrow$ perpendicular distance of $(x, y)$ to line segment $L$
    \STATE \algorithmicif\ $(x,y)$ to right of $L$
    \STATE \algorithmicthen\ $d = d_{\text{line}} + f1*p$\
    \STATE \algorithmicelse\ $d = d_{\text{line}} - f1*p$\
    \STATE left leg velocity $\omega_l \leftarrow \omega_{\text{nom}} - d*f2$
    \STATE right leg velocity $\omega_r \leftarrow \omega_{\text{nom}} + d*f2$
    \STATE \textbf{Outputs}: leg PID velocity setpoints $\omega_l$ and $\omega_r$
\end{algorithmic}
\end{algorithm}
